WPMixer: Efficient Multi-Resolution Mixing for Long-Term Time Series Forecasting

Time series forecasting is crucial for various applications, such as weather forecasting, power load forecasting, and financial analysis. In recent studies, MLP-mixer models for time series forecasting have been shown as a promising alternative to transformer-based models. However, the performance of these models is still yet to reach its potential. In this paper, we propose Wavelet Patch Mixer (WPMixer), a novel MLP-based model, for long-term time series forecasting, which leverages the benefits of patching, multi-resolution wavelet decomposition, and mixing. Our model is based on three key components: (i) multi-resolution wavelet decomposition, (ii) patching and embedding, and (iii) MLP mixing. Multi-resolution wavelet decomposition efficiently extracts information in both the frequency and time domains. Patching allows the model to capture an extended history with a look-back window and enhances capturing local information while MLP mixing incorporates global information. Our model significantly outperforms state-of-the-art MLP-based and transformer-based models for long-term time series forecasting in a computationally efficient way, demonstrating its efficacy and potential for practical applications.

==> main_result_no_need_.tex <==

\begin{table*}[!htb]
    \fontsize{9}{8}\selectfont
    \begin{tabularx}{\textwidth}{@{}cccccccccccccccccc@{}}
        \multicolumn{2}{c}{\multirow{2}{*}{Models}} & \multicolumn{2}{c}{WPMixer} & \multicolumn{2}{c}{TimeMixer*} & \multicolumn{2}{c}{PatchTST} & \multicolumn{2}{c}{TSMixer} & \multicolumn{2}{c}{TimesNet} & \multicolumn{2}{c}{Crossformer*} & \multicolumn{2}{c}{FiLM*} & \multicolumn{2}{c}{Dlinear*} \\
        \multicolumn{2}{c}{} & \multicolumn{2}{c}{(Ours)} & \multicolumn{2}{c}{2024} & \multicolumn{2}{c}{2023} & \multicolumn{2}{c}{2023} & \multicolumn{2}{c}{2022} & \multicolumn{2}{c}{2023} & \multicolumn{2}{c}{2022a} & \multicolumn{2}{c}{2023} \\
        \toprule
        \multicolumn{2}{c}{Metric} & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\
        \midrule
        \multirow{5}{*}{ETTh1} & 96 & \textbf{0.347} & \textbf{0.383} & \underline{0.361} & \underline{0.390} & 0.370 & 0.400 & \underline{0.361} & 0.392 & 0.384 & 0.402 & 0.418 & 0.438 & 0.422 & 0.432 & 0.375 & 0.399 \\
         & 192 & \textbf{0.381} & \textbf{0.408} & 0.409 & \underline{0.414} & 0.413 & 0.429 & \underline{0.404} & 0.418 & 0.436 & 0.429 & 0.539 & 0.517 & 0.462 & 0.458 & 0.405 & 0.416 \\
         & 336 & \textbf{0.382} & \textbf{0.412} & 0.430 & \underline{0.429} & 0.422 & 0.440 & \underline{0.420} & 0.431 & 0.491 & 0.469 & 0.709 & 0.638 & 0.501 & 0.483 & 0.439 & 0.443 \\
         & 720 & \textbf{0.405} & \textbf{0.432} & \underline{0.445} & \underline{0.460} & 0.447 & 0.468 & 0.463 & 0.472 & 0.521 & 0.500 & 0.733 & 0.636 & 0.544 & 0.526 & 0.472 & 0.490 \\
         \cmidrule{2-18}
         & Avg & \textbf{0.379} & \textbf{0.409} & \underline{0.411} & \underline{0.423} & 0.413 & 0.434 & 0.412 & 0.428 & 0.458 & 0.450 & 0.600 & 0.557 & 0.482 & 0.475 & 0.423 & 0.437 \\
         \midrule
        \multirow{5}{*}{ETTh2} & 96 & \textbf{0.253} & \textbf{0.328} & \underline{0.271} & \underline{0.330} & 0.274 & 0.337 & 0.274 & 0.341 & 0.340 & 0.374 & 0.425 & 0.463 & 0.323 & 0.370 & 0.289 & 0.353 \\
         & 192 & \textbf{0.303} & \textbf{0.364} & \underline{0.317} & 0.402 & 0.341 & \underline{0.382} & 0.339 & 0.385 & 0.402 & 0.414 & 0.473 & 0.500 & 0.391 & 0.415 & 0.383 & 0.418 \\
         & 336 & \textbf{0.305} & \textbf{0.371} & 0.332 & 0.396 & \underline{0.329} & \underline{0.384} & 0.361 & 0.406 & 0.452 & 0.452 & 0.581 & 0.562 & 0.415 & 0.440 & 0.448 & 0.465 \\
         & 720 & \underline{0.373} & \underline{0.417} & \textbf{0.342} & \textbf{0.408} & 0.379 & 0.422 & 0.445 & 0.470 & 0.462 & 0.468 & 0.775 & 0.665 & 0.441 & 0.459 & 0.605 & 0.551 \\
          \cmidrule{2-18}
         & Avg & \textbf{0.309} & \textbf{0.370} & \underline{0.316} & 0.384 & 0.331 & \underline{0.381} & 0.355 & 0.401 & 0.414 & 0.427 & 0.564 & 0.548 & 0.393 & 0.421 & 0.431 & 0.447 \\
         \midrule
        \multirow{5}{*}{ETTm1} & 96 & \textbf{0.275} & \textbf{0.333} & 0.291 & 0.340 & 0.293 & 0.346 & \underline{0.285} & \underline{0.339} & 0.338 & 0.375 & 0.361 & 0.403 & 0.302 & 0.345 & 0.299 & 0.343 \\
         & 192 & \textbf{0.319} & \textbf{0.362} & \underline{0.327} & \underline{0.365} & 0.333 & 0.370 & \underline{0.327} & \underline{0.365} & 0.374 & 0.387 & 0.387 & 0.422 & 0.338 & 0.368 & 0.335 & \underline{0.365} \\
         & 336 & \textbf{0.347} & 0.384 & 0.360 & \textbf{0.381} & 0.369 & 0.392 & \underline{0.356} & \underline{0.382} & 0.410 & 0.411 & 0.605 & 0.572 & 0.373 & 0.388 & 0.369 & 0.386 \\
         & 720 & \textbf{0.403} & \textbf{0.414} & \underline{0.415} & 0.417 & 0.416 & 0.420 & 0.419 & \textbf{0.414} & 0.478 & 0.450 & 0.703 & 0.645 & 0.420 & 0.420 & 0.425 & 0.421 \\
          \cmidrule{2-18}
         & Avg & \textbf{0.336} & \textbf{0.373} & 0.348 & \underline{0.375} & 0.353 & 0.382 & \underline{0.347} & \underline{0.375} & 0.400 & 0.406 & 0.514 & 0.510 & 0.358 & 0.380 & 0.357 & 0.379 \\
         \midrule
        \multirow{5}{*}{ETTm2} & 96 & \textbf{0.159} & \textbf{0.246} & 0.164 & 0.254 & 0.166 & 0.256 & \underline{0.163} & \underline{0.252} & 0.187 & 0.267 & 0.275 & 0.358 & 0.165 & 0.256 & 0.167 & 0.260 \\
         & 192 & \textbf{0.214} & \textbf{0.286} & 0.223 & 0.295 & 0.223 & 0.296 & \underline{0.216} & \underline{0.290} & 0.249 & 0.309 & 0.345 & 0.400 & 0.222 & 0.296 & 0.224 & 0.303 \\
         & 336 & \textbf{0.266} & \textbf{0.322} & 0.279 & 0.330 & 0.274 & 0.329 & \underline{0.268} & \underline{0.324} & 0.321 & 0.351 & 0.657 & 0.528 & 0.277 & 0.333 & 0.281 & 0.342 \\
         & 720 & \textbf{0.344} & \textbf{0.374} & \underline{0.359} & \underline{0.383} & 0.362 & 0.385 & 0.420 & 0.422 & 0.408 & 0.403 & 1.208 & 0.753 & 0.371 & 0.389 & 0.397 & 0.421 \\
          \cmidrule{2-18}
         & Avg & \textbf{0.246} & \textbf{0.307} & \underline{.256} & \underline{0.315} & \underline{0.256} & 0.317 & 0.267 & 0.322 & 0.291 & 0.333 & 0.621 & 0.510 & 0.259 & 0.319 & 0.267 & 0.332 \\
         \midrule
        \multirow{5}{*}{Weather} & 96 & \textbf{0.141} & \textbf{0.188} & 0.147 & \underline{0.197} & 0.149 & 0.198 & \underline{0.145} & 0.198 & 0.172 & 0.220 & 0.232 & 0.302 & 0.199 & 0.262 & 0.176 & 0.237 \\
         & 192 & \textbf{0.185} & \textbf{0.229} & \underline{0.189} & \underline{0.239} & 0.194 & 0.241 & 0.191 & 0.242 & 0.219 & 0.261 & 0.371 & 0.410 & 0.228 & 0.288 & 0.220 & 0.282 \\
         & 336 & \textbf{0.236} & \textbf{0.271} & \underline{0.241} & \underline{0.280} & 0.245 & 0.282 & 0.242 & \underline{0.280} & 0.280 & 0.306 & 0.495 & 0.515 & 0.267 & 0.323 & 0.265 & 0.319 \\
         & 720 & \textbf{0.307} & \textbf{0.321} & \underline{0.310} & \underline{0.330} & 0.314 & 0.334 & 0.320 & 0.336 & 0.365 & 0.359 & 0.526 & 0.542 & 0.319 & 0.361 & 0.323 & 0.362 \\
          \cmidrule{2-18}
         & Avg & \textbf{0.217} & \textbf{0.252} & \underline{0.222} & \underline{0.262} & 0.226 & 0.264 & 0.225 & 0.264 & 0.259 & 0.287 & 0.406 & 0.442 & 0.253 & 0.309 & 0.246 & 0.300 \\
         \midrule
        \multirow{5}{*}{Electricity} & 96 & \textbf{0.128} & \textbf{0.222} & \underline{0.129} & 0.224 & \underline{0.129} & \textbf{0.222} & 0.131 & 0.229 & 0.168 & 0.272 & 0.150 & 0.251 & 0.154 & 0.267 & 0.140 & 0.237 \\
         & 192 & \underline{0.145} & \underline{0.237} & \textbf{0.140} & \textbf{0.220} & 0.147 & 0.240 & 0.151 & 0.246 & 0.184 & 0.289 & 0.161 & 0.260 & 0.164 & 0.258 & 0.153 & 0.249 \\
         & 336 & \textbf{0.161} & \underline{0.256} & \textbf{0.161} & \textbf{0.255} & 0.163 & 0.259 & \textbf{0.161} & 0.261 & 0.198 & 0.300 & 0.182 & 0.281 & 0.188 & 0.283 & 0.169 & 0.267 \\
         & 720 & \underline{0.196} & \textbf{0.287} & \textbf{0.194} & \textbf{0.287} & 0.197 & 0.290 & 0.197 & 0.293 & 0.220 & 0.320 & 0.251 & 0.339 & 0.236 & 0.332 & 0.203 & 0.301 \\
          \cmidrule{2-18}
         & Avg & \underline{0.158} & \underline{0.251} & \textbf{0.156} & \textbf{0.246} & 0.159 & 0.253 & 0.160 & 0.257 & 0.192 & 0.295 & 0.186 & 0.283 & 0.186 & 0.285 & 0.166 & 0.264 \\
         \midrule
        \multirow{5}{*}{Traffic} & 96 & \textbf{0.354} & \textbf{0.246} & \underline{0.360} & \underline{0.249} & \underline{0.360} & \underline{0.249} & 0.376 & 0.264 & 0.593 & 0.321 & 0.514 & 0.267 & 0.416 & 0.294 & 0.410 & 0.282 \\
         & 192 & \textbf{0.371} & 0.253 & \underline{0.375} & \textbf{0.250} & 0.379 & 0.256 & 0.397 & 0.277 & 0.617 & 0.336 & 0.549 & \underline{0.252} & 0.408 & 0.288 & 0.423 & 0.287 \\
         & 336 & \underline{0.387} & \underline{0.267} & \textbf{0.385} & 0.270 & 0.392 & \textbf{0.264} & 0.413 & 0.290 & 0.629 & 0.336 & 0.530 & 0.300 & 0.425 & 0.298 & 0.436 & 0.296 \\
         & 720 & \underline{0.431} & 0.289 & \textbf{0.430} & \textbf{0.281} & 0.432 & \underline{0.286} & 0.444 & 0.306 & 0.640 & 0.350 & 0.573 & 0.313 & 0.520 & 0.353 & 0.466 & 0.315 \\
          \cmidrule{2-18}
         & Avg & \textbf{0.386} & \underline{0.264} & \underline{0.387} & \textbf{0.262} & 0.391 & \underline{0.264} & 0.408 & 0.284 & 0.620 & 0.336 & 0.542 & 0.283 & 0.442 & 0.308 & 0.434 & 0.295 \\
         \midrule
        \multicolumn{1}{l}{} & \multicolumn{1}{l}{1st Count:} & 29 & 26 & 7 & 9 & 0 & 2 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
        \bottomrule
    \end{tabularx}
    \caption{Multivariate long-term forecasting results. The length of the look-back window is a hyperparameter. The results of the models marked with $*$ are taken from \cite{c:timemixer}; other results are taken from the corresponding papers.}
    \label{tab:search_result}
\end{table*}

==> table_ablation_no_need_.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[!htb]
\centering
\fontsize{9}{9}\selectfont
\begin{tabularx}{\textwidth}{@{}ccllllllllllllcl@{}}
\toprule
\multicolumn{2}{r}{Case} & \multicolumn{1}{c}{\textbf{I}} & \multicolumn{1}{c}{\textbf{II}} & \multicolumn{1}{c}{\textbf{III}} & \multicolumn{1}{c}{\textbf{IV}} & \multicolumn{1}{c}{\textbf{V}} & \multicolumn{1}{c}{\textbf{VI}} & \multicolumn{1}{c}{\textbf{VII}} & \multicolumn{1}{c}{\textbf{VIII}} & \multicolumn{1}{c}{\textbf{IX}} & \multicolumn{1}{c}{\textbf{X}} & \multicolumn{1}{c}{\textbf{XI}} & \multicolumn{1}{c}{\textbf{XII}} & \textbf{XIII} & \multicolumn{1}{c}{\textbf{XIV}} \\ \midrule
\multicolumn{2}{r}{Patch} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & $\checkmark$ & \multicolumn{1}{c}{$\checkmark$} \\
\multicolumn{2}{r}{Embedding} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & $\checkmark$ & \multicolumn{1}{c}{$\checkmark$} \\
\multicolumn{2}{r}{Decomposition} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\times$} & $\checkmark$ & \multicolumn{1}{c}{$\times$} \\
\multicolumn{2}{r}{Mixing with Feed Forward} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} \\
\multicolumn{2}{r}{Mixing without Feed Forward} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & \multicolumn{1}{c}{$\times$} & $\checkmark$ & \multicolumn{1}{c}{$\checkmark$} \\
\multicolumn{2}{r}{Head} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & \multicolumn{1}{c}{$\checkmark$} & $\checkmark$ & \multicolumn{1}{c}{$\checkmark$} \\ \midrule
\multirow{4}{*}{\textbf{ETTh1}} & \textbf{96} & 0.347 & 0.351 & 0.349 & 0.353 & 0.343 & 0.350 & 0.357 & 0.359 & 0.359 & 0.359 & 0.359 & 0.359 & 0.348 & 0.349 \\
 & \textbf{192} & 0.381 & 0.392 & 0.383 & 0.391 & 0.380 & 0.386 & 0.395 & 0.396 & 0.399 & 0.398 & 0.398 & 0.399 & 0.384 & 0.394 \\
 & \textbf{336} & 0.382 & 0.391 & 0.384 & 0.392 & 0.378 & 0.394 & 0.395 & 0.403 & 0.399 & 0.406 & 0.401 & 0.407 & 0.383 & 0.393 \\
 & \textbf{720} & 0.405 & 0.419 & 0.419 & 0.432 & 0.409 & 0.432 & 0.431 & 0.439 & 0.442 & 0.446 & 0.440 & 0.446 & 0.395 & 0.430 \\ \cmidrule{3-16}
\textbf{} & \textbf{Avg.} & 0.379 & 0.388 & 0.384 & 0.392 & 0.378 & 0.390 & 0.394 & 0.399 & 0.400 & 0.403 & 0.400 & 0.403 & \multicolumn{1}{l}{0.377} & 0.392 \\ \midrule
\multirow{4}{*}{\textbf{ETTh2}} & \textbf{96} & 0.253 & 0.254 & 0.260 & 0.259 & 0.254 & 0.257 & 0.253 & 0.253 & 0.253 & 0.250 & 0.252 & 0.254 & 0.257 & 0.257 \\
 & \textbf{192} & 0.303 & 0.310 & 0.311 & 0.315 & 0.306 & 0.313 & 0.304 & 0.308 & 0.304 & 0.305 & 0.303 & 0.305 & 0.310 & 0.312 \\
 & \textbf{336} & 0.305 & 0.307 & 0.315 & 0.323 & 0.314 & 0.317 & 0.313 & 0.312 & 0.320 & 0.318 & 0.316 & 0.316 & 0.312 & 0.311 \\
 & \textbf{720} & 0.373 & 0.374 & 0.378 & 0.402 & 0.381 & 0.394 & 0.375 & 0.374 & 0.383 & 0.386 & 0.379 & 0.381 & 0.378 & 0.376 \\ \cmidrule{3-16}
\textbf{} & \textbf{Avg.} & 0.308 & 0.311 & 0.316 & 0.325 & 0.314 & 0.320 & 0.311 & 0.312 & 0.315 & 0.315 & 0.312 & 0.314 & \multicolumn{1}{l}{0.314} & 0.314 \\ \midrule
\multirow{4}{*}{\textbf{ETTm1}} & \textbf{96} & 0.275 & 0.282 & 0.283 & 0.285 & 0.283 & 0.288 & 0.302 & 0.302 & 0.303 & 0.302 & 0.303 & 0.302 & 0.283 & 0.287 \\
 & \textbf{192} & 0.319 & 0.325 & 0.319 & 0.324 & 0.321 & 0.327 & 0.334 & 0.333 & 0.335 & 0.335 & 0.334 & 0.335 & 0.318 & 0.325 \\
 & \textbf{336} & 0.347 & 0.351 & 0.347 & 0.354 & 0.350 & 0.354 & 0.362 & 0.363 & 0.365 & 0.364 & 0.364 & 0.364 & 0.346 & 0.351 \\
 & \textbf{720} & 0.403 & 0.398 & 0.407 & 0.418 & 0.403 & 0.401 & 0.415 & 0.417 & 0.419 & 0.418 & 0.418 & 0.418 & 0.410 & 0.403 \\ \cmidrule{3-16}
\textbf{} & \textbf{Avg.} & 0.336 & 0.339 & 0.339 & 0.345 & 0.339 & 0.343 & 0.353 & 0.354 & 0.356 & 0.355 & 0.355 & 0.355 & \multicolumn{1}{l}{0.339} & 0.342 \\ \midrule
\multirow{4}{*}{\textbf{ETTm2}} & \textbf{96} & 0.159 & 0.161 & 0.162 & 0.162 & 0.161 & 0.162 & 0.161 & 0.161 & 0.162 & 0.161 & 0.161 & 0.161 & 0.161 & 0.161 \\
 & \textbf{192} & 0.214 & 0.215 & 0.218 & 0.218 & 0.215 & 0.215 & 0.216 & 0.216 & 0.216 & 0.217 & 0.217 & 0.217 & 0.215 & 0.215 \\
 & \textbf{336} & 0.266 & 0.267 & 0.270 & 0.269 & 0.268 & 0.266 & 0.272 & 0.272 & 0.272 & 0.272 & 0.271 & 0.271 & 0.267 & 0.266 \\
 & \textbf{720} & 0.344 & 0.346 & 0.350 & 0.347 & 0.343 & 0.347 & 0.357 & 0.357 & 0.352 & 0.357 & 0.354 & 0.357 & 0.346 & 0.350 \\ \cmidrule{3-16}
\textbf{} & \textbf{Avg.} & 0.245 & 0.247 & 0.250 & 0.249 & 0.247 & 0.248 & 0.252 & 0.252 & 0.251 & 0.252 & 0.251 & 0.252 & \multicolumn{1}{l}{0.247} & 0.248 \\ \bottomrule
\end{tabularx}
\caption{ Detailed contribution of each module of our model. MSE (Meas Square Error) values for multivariate long-term forecasting with input length equal to 512 and prediction length equal to 96, 192, 336, and 720. ($\checkmark$) mark refers to the presence of that module, where ($\times$) mark refers to the absence of that module.}
\label{tab:ablation}
\end{table*}

==> table_ablation_short_result_no_need_.tex <==
\begin{table}[!htb]
    \centering
    \fontsize{9}{6}\selectfont
    \begin{tabularx}{\columnwidth}{c|cccccc|c|c|c|c}
        \toprule
         & \multicolumn{6}{c|}{Modules} & \begin{sideways}ETTh1\end{sideways} & \begin{sideways}ETTh2\end{sideways} & \begin{sideways}ETTm1\end{sideways} & \begin{sideways}ETTm2\end{sideways} \\ \midrule
        Case & $D$ & $P$ & $E$ & $P_x$ & $E_x$ & $H$ & MSE & MSE & MSE & MSE \\ \midrule
        I & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 0.379 & 0.308 & 0.336 & 0.245 \\
        II & $\times$ & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 0.388 & 0.311 & 0.339 & 0.247 \\
        III & \checkmark & $\times$ & $\times$ & \checkmark & \checkmark & \checkmark & 0.384 & 0.316 & 0.339 & 0.250 \\
        IV & $\times$ & $\times$ & $\times$ & \checkmark & \checkmark & \checkmark & 0.392 & 0.325 & 0.345 & 0.249 \\
        V & \checkmark & \checkmark & $\times$ & \checkmark & \checkmark & \checkmark & 0.378 & 0.314 & 0.339 & 0.247 \\
        VI & $\times$ & \checkmark & $\times$ & \checkmark & \checkmark & \checkmark & 0.390 & 0.320 & 0.343 & 0.248 \\
        VII & \checkmark & \checkmark & \checkmark & $\times$ & $\times$ & \checkmark & 0.394 & 0.311 & 0.353 & 0.252 \\
        VIII & $\times$ & \checkmark & \checkmark & $\times$ & $\times$ & \checkmark & 0.399 & 0.312 & 0.354 & 0.252 \\
        IX & \checkmark & $\times$ & $\times$ & $\times$ & $\times$ & \checkmark & 0.400 & 0.315 & 0.356 & 0.251 \\
        X & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & \checkmark & 0.403 & 0.315 & 0.355 & 0.252 \\
        XI & \checkmark & \checkmark & $\times$ & $\times$ & $\times$ & \checkmark & 0.400 & 0.312 & 0.355 & 0.251 \\
        XII & $\times$ & \checkmark & $\times$ & $\times$ & $\times$ & \checkmark & 0.403 & 0.314 & 0.355 & 0.252 \\
        XIII & \checkmark & \checkmark & \checkmark & $\times$ & \checkmark & \checkmark & 0.377 & 0.314 & 0.339 & 0.247 \\
        XIV & $\times$ & \checkmark & \checkmark & $\times$ & \checkmark & \checkmark & 0.392 & 0.314 & 0.342 & 0.248 \\ \bottomrule
    \end{tabularx}
    \caption{Contribution of each module in WPMixer. $D$, $P$, $E$, $P_x$, $E_x$, and $H$ refer to the decomposition, patch, embedding, patch mixer, embedding mixer, and head modules, respectively. Look-back window is set to 512. Results are averaged over the prediction lengths 96, 192, 336, and 720.}
    \label{tab:ablation_result_short}
\end{table}

==> table_datasets_no_need_.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[htbp!]
    \centering
    \fontsize{9}{6}\selectfont
    \begin{tabularx}{\columnwidth}{@{}c|c|c|c@{}}
    \toprule
        Dataset & Variates & Dataset Size & Freq. \\ \midrule
        ETTh1, ETTh2 & 7 & (8545, 2881, 2881) & Hourly \\
        ETTm1, ETTm2 & 7 & (34465, 11521, 11521) & 15 min \\
        Weather & 21 & (36792, 5271, 10540) & 10 min \\
        Electricity & 321 & (18317, 2633, 5261) & Hourly \\
        Traffic & 862 & (12185, 1757, 3509) & Hourly \\ \bottomrule
    \end{tabularx}
    \caption{Specifications of the datasets. Dataset size refers to the training, validation, and testing dataset sizes.}
    \label{tab:dataset_details}
\end{table}

==> table_full_gflops_no_need_.tex <==

\begin{table}[]
\begin{tabularx}{\columnwidth}{lllllllll}
 &  &  & \multicolumn{3}{l}{WPMixer} & \multicolumn{3}{l}{TimeMixer} \\
 & T & d & MSE & MAE & GFLOPs & MSE & MAE & GFLOPs \\
\multirow{20}{*}{ETTh1} & \multirow{5}{*}{96} & 16 & 0.370 & 0.390 & 0.210 & 0.375 & 0.400 & 2.774 \\
 &  & 32 & 0.368 & 0.390 & 0.584 &  &  &  \\
 &  & 64 & 0.369 & 0.388 & 1.617 &  &  &  \\
 &  & 128 & 0.365 & 0.389 & 4.926 &  &  &  \\
 &  & 256 & 0.366 & 0.391 & 34.035 &  &  &  \\
 & \multirow{5}{*}{192} & 16 & 0.424 & 0.420 & 0.226 & 0.429 & 0.421 & 3.281 \\
 &  & 32 & 0.427 & 0.419 & 0.826 &  &  &  \\
 &  & 64 & 0.427 & 0.421 & 1.343 &  &  &  \\
 &  & 128 & 0.422 & 0.420 & 10.515 &  &  &  \\
 &  & 256 & 0.418 & 0.419 & 18.215 &  &  &  \\
 & \multirow{5}{*}{336} & 16 & 0.462 & 0.433 & 0.211 & 0.484 & 0.458 & 4.040 \\
 &  & 32 & 0.463 & 0.433 & 0.811 &  &  &  \\
 &  & 64 & 0.450 & 0.436 & 2.163 &  &  &  \\
 &  & 128 & 0.453 & 0.436 & 12.082 &  &  &  \\
 &  & 256 & 0.465 & 0.439 & 41.055 &  &  &  \\
 & \multirow{5}{*}{720} & 16 & 0.455 & 0.449 & 0.481 & 0.498 & 0.482 & 6.066 \\
 &  & 32 & 0.452 & 0.448 & 1.244 &  &  &  \\
 &  & 64 & 0.451 & 0.443 & 4.725 &  &  &  \\
 &  & 128 & 0.449 & 0.445 & 12.370 &  &  &  \\
 &  & 256 & 0.458 & 0.446 & 19.101 &  &  & 
\end{tabularx}
\caption{}
\label{tab:full_gflops}
\end{table}

==> table_gflops_no_need_.tex <==
\begin{table}[htbp!]
    \centering
    \fontsize{9}{7}\selectfont
    \begin{tabularx}{\columnwidth}{@{}c|c|ccc|ccc@{}}
        \toprule
         &  & \multicolumn{3}{c|}{WPMixer} & \multicolumn{3}{c}{TimeMixer} \\ \midrule
         & T & MSE & MAE & GFLOPs & MSE & MAE & GFLOPs \\ \midrule
        \multirow{4}{*}{\begin{sideways}ETTh1\end{sideways}} & 96 & 0.370 & 0.390 & 0.210 & 0.375 & 0.400 & 2.774 \\
         & 192 & 0.424 & 0.420 & 0.226 & 0.429 & 0.421 & 3.281 \\
         & 336 & 0.462 & 0.433 & 0.211 & 0.484 & 0.458 & 4.040 \\
         & 720 & 0.455 & 0.449 & 0.481 & 0.498 & 0.482 & 6.066 \\ \bottomrule
    \end{tabularx}
    
    \caption{WPMixer is ten folds more efficient for $d=16$.}
    \label{tab:table_gflops}
\end{table}

==> table_hyperparameters_no_need_.tex <==
\begin{table*}[!htbp]
    \fontsize{9}{6}\selectfont
    \centering
    \begin{tabularx}{\textwidth}{@{}c|c|c|c|c|c|c|c|c|c|c|c|c|c|c@{}}
        \toprule
         & Pred len & Look back & Initial lr & Batch & $\psi$ & $m$ & $t_f$ & $d_f$ & Mixer d/o & embed d/o & Patch & Stride & $d$ & epochs \\ \midrule
        \multirow{4}{*}{ETTh1} & 96 & 512 & 0.00024 & 256 & db2 & 2 & 5 & 8 & 0.4 & 0.1 & 16 & 8 & 256 & 30 \\
         & 192 & 512 & 0.0002 & 256 & db3 & 2 & 5 & 5 & 0.05 & 0.2 & 16 & 8 & 256 & 30 \\
         & 336 & 512 & 0.00013 & 256 & db2 & 1 & 3 & 3 & 0 & 0.4 & 16 & 8 & 256 & 30 \\
         & 720 & 512 & 0.00024 & 256 & db2 & 1 & 5 & 3 & 0.2 & 0.4 & 16 & 8 & 128 & 30 \\  \midrule
        \multirow{4}{*}{ETTh2} & 96 & 512 & 0.00047 & 256 & db2 & 2 & 5 & 5 & 0 & 0.1 & 16 & 8 & 256 & 30 \\
         & 192 & 512 & 0.00029 & 256 & db2 & 3 & 3 & 8 & 0 & 0 & 16 & 8 & 256 & 30 \\
         & 336 & 512 & 0.00062 & 256 & db2 & 5 & 5 & 3 & 0.1 & 0.1 & 16 & 8 & 128 & 30 \\
         & 720 & 512 & 0.00081 & 256 & db2 & 5 & 5 & 5 & 0.4 & 0 & 16 & 8 & 128 & 30 \\  \midrule
        \multirow{4}{*}{ETTm1} & 96 & 512 & 0.00128 & 256 & db2 & 1 & 5 & 3 & 0.4 & 0.2 & 48 & 24 & 256 & 80 \\
         & 192 & 512 & 0.00242 & 256 & db3 & 1 & 3 & 7 & 0.4 & 0.05 & 48 & 24 & 128 & 80 \\
         & 336 & 512 & 0.00159 & 256 & db5 & 1 & 7 & 7 & 0.4 & 0 & 48 & 24 & 256 & 80 \\
         & 720 & 512 & 0.00201 & 256 & db5 & 4 & 3 & 8 & 0.4 & 0.05 & 48 & 24 & 128 & 80 \\  \midrule
        \multirow{4}{*}{ETTm2} & 96 & 512 & 0.00077 & 256 & bior3.1 & 1 & 3 & 8 & 0.4 & 0 & 48 & 24 & 256 & 80 \\
         & 192 & 512 & 0.00028 & 256 & db2 & 1 & 3 & 7 & 0.2 & 0.1 & 48 & 24 & 256 & 80 \\
         & 336 & 512 & 0.00023 & 256 & db2 & 1 & 3 & 5 & 0.4 & 0 & 48 & 24 & 256 & 80 \\
         & 720 & 512 & 0.00104 & 256 & db2 & 1 & 3 & 8 & 0.4 & 0 & 48 & 24 & 256 & 80 \\  \midrule
        \multirow{4}{*}{Weather} & 96 & 512 & 0.00091 & 32 & db3 & 2 & 3 & 7 & 0.4 & 0.1 & 16 & 8 & 256 & 60 \\
         & 192 & 512 & 0.00138 & 64 & db3 & 1 & 3 & 7 & 0.4 & 0 & 16 & 8 & 128 & 60 \\
         & 336 & 512 & 0.00061 & 32 & db3 & 2 & 7 & 7 & 0.4 & 0.4 & 16 & 8 & 128 & 60 \\
         & 720 & 512 & 0.00223 & 128 & db2 & 3 & 7 & 5 & 0.1 & 0.4 & 16 & 8 & 256 & 60 \\  \midrule
        \multirow{4}{*}{Electricity} & 96 & 512 & 0.00328 & 32 & sym3 & 2 & 3 & 5 & 0.1 & 0 & 16 & 8 & 32 & 100 \\
         & 192 & 512 & 0.00049 & 32 & coif5 & 3 & 7 & 5 & 0.1 & 0.05 & 16 & 8 & 32 & 100 \\
         & 336 & 512 & 0.00251 & 32 & sym4 & 1 & 5 & 7 & 0.2 & 0.05 & 16 & 8 & 32 & 100 \\
         & 720 & 512 & 0.00198 & 32 & db2 & 2 & 7 & 8 & 0.1 & 0 & 16 & 8 & 32 & 100 \\  \midrule
        \multirow{4}{*}{Traffic} & 96 & 1200 & 0.00104 & 16 & db3 & 1 & 3 & 5 & 0.05 & 0.05 & 16 & 8 & 16 & 60 \\
         & 192 & 1200 & 0.00057 & 16 & db3 & 1 & 3 & 5 & 0.05 & 0 & 16 & 8 & 32 & 60 \\
         & 336 & 1200 & 0.00103 & 16 & bior3.1 & 1 & 7 & 7 & 0 & 0.1 & 16 & 8 & 32 & 60 \\
         & 720 & 1200 & 0.0015 & 16 & db3 & 1 & 7 & 3 & 0.05 & 0.2 & 16 & 8 & 32 & 60 \\ \bottomrule
    \end{tabularx}
    \caption{Comprehensive hyper-parameter settings for the multi-variate long-term forecasting task, optimized using Optuna. The hyper-parameters Wavelet $\psi$ and decomposition level $m$ are utilized in Equation \ref{eq:pmd1}. Expansion factors $t_f$ and $d_f$ are incorporated in Equations \ref{eq:mix2} and \ref{eq:mix4}, respectively. The hyper-parameter $d$ is applied in Equation \ref{eq:embed}. "Mixer d/o" and "Embed d/o" denote the distinct dropouts employed in the Mixer module and the Embedding Layer. Learning rate is gradually reduced in the training using the formula, $lr := lr \times 0.9^{(epoch -3)}$} 
    \label{tab:hyperparameters_list}
\end{table*}


==> table_hyperparameters_range_no_need_.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[!htbp]
    \centering
    \fontsize{9}{7}\selectfont
    \begin{tabular}{@{}c|c|c|c|c|c@{}}
        \toprule
         & ETTh & ETTm & Weather & Electricity & Traffic \\ \midrule
        Batch & 256 & 256 & 32, 64, 128 & 32 & 16 \\ \midrule
        $d$ & 128, 256 & 128, 256 & 128, 256 & 16, 32 & 16, 32 \\ \midrule
        Look back window& \multicolumn{5}{c}{96, 336, 512, 1024, 1200} \\ \midrule
        Initial lr & \multicolumn{5}{c}{max 0.01, min 0.00001} \\ \midrule
        $\psi$ & \multicolumn{5}{c}{db2,   db3, db5, sym2, sym3, sym4, sym5, coif4, coif5, bior3.1, bior3.5} \\ \midrule
        $m$ & \multicolumn{5}{c}{1, 2, 3, 4, 5} \\ \midrule
        $t_f$ & \multicolumn{5}{c}{3, 5, 7, 9} \\ \midrule
        $d_f$ & \multicolumn{5}{c}{3, 5, 7, 8, 9} \\ \midrule
        Mixer Dropout & \multicolumn{5}{c}{0.0, 0.05, 0.1, 0.2, 0.4} \\ \midrule
        Embedding Layer Dropout & \multicolumn{5}{c}{0.0, 0.05, 0.1, 0.2, 0.4} \\ \midrule
        Patch-Stride & \multicolumn{5}{c}{16-8, 32-16, 48-24} \\ \bottomrule
    \end{tabular}
    \caption{Hyperparameters search space. Wavelet type db*, sym*, coif*, and bior* refer to the Daubechies, Symlets, Coiflets, and Biorthogonal wavelet family, respectively.}
    \label{tab:hyper_parameters_range}
\end{table*}

==> table_mse_vs_smoothL1_no_need_.tex <==

%\begin{table}[!htbp]
%\centering
%\fontsize{9}{9}\selectfont
%\begin{tabularx}{\columnwidth}{@{}cccc|cc@{}}
% &  & \multicolumn{4}{c}{WPMixer} \\ \toprule
% &  & \multicolumn{2}{c}{MSE Loss} & \multicolumn{2}{|c}{SmoothL1Loss} \\ \cmidrule{3-6}
%data & Pred len & MSE & MAE & MSE & MAE \\ \midrule
%\multirow{4}{*}{ETTm2} & 96 & 0.165 & 0.257 & 0.159 & 0.246 \\
% & 192 & 0.219 & 0.291 & 0.214 & 0.286 \\
% & 336 & 0.271 & 0.327 & 0.266 & 0.322 \\
% & 720 & 0.349 & 0.384 & 0.344 & 0.374 \\ \midrule
%\multirow{4}{*}{ETTh2} & 96 & 0.251 & 0.327 & 0.253 & 0.328 \\
% & 192 & 0.308 & 0.365 & 0.303 & 0.364 \\
% & 336 & 0.306 & 0.373 & 0.305 & 0.371 \\
% & 720 & 0.374 & 0.419 & 0.373 & 0.417 \\ \bottomrule
%\end{tabularx}
%\caption{Model's performance with criterion: $MSE loss$, and $SmoothL1Loss$.}
%\label{tab:mse_vs_smoothL1}
%\end{table}

\begin{table}[!htbp]
    \centering
    \fontsize{9}{6}\selectfont
    \begin{tabularx}{\columnwidth}{c|cccc|cccc}
        \toprule
         & \multicolumn{4}{c|}{ETTm2} & \multicolumn{4}{c}{ETTh2} \\ \midrule
         & \multicolumn{2}{c}{$MSEloss$} & \multicolumn{2}{c|}{$SmoothL1$} & \multicolumn{2}{c}{$MSEloss$} & \multicolumn{2}{c}{$SmoothL1$} \\ \midrule
        T & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\ \midrule
        96 & 0.165 & 0.257 & 0.159 & 0.246 & 0.251 & 0.327 & 0.253 & 0.328 \\
        192 & 0.219 & 0.291 & 0.214 & 0.286 & 0.308 & 0.365 & 0.303 & 0.364 \\
        336 & 0.271 & 0.327 & 0.266 & 0.322 & 0.306 & 0.373 & 0.305 & 0.371 \\
        720 & 0.349 & 0.384 & 0.344 & 0.374 & 0.374 & 0.419 & 0.373 & 0.417 \\ \bottomrule
    \end{tabularx}
    \caption{$SmoothL1$ loss vs. $MSE$ loss for training.}
    \label{tab:mse_vs_smoothL1}
\end{table}

==> table_robustness_no_need_.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[!htb]
    \fontsize{9}{9}\selectfont
    \begin{tabularx}{\columnwidth}{@{}c|cc|cc@{}}
        \toprule
        \multirow{2}{*}{} & \multicolumn{2}{c|}{WPMixer} & \multicolumn{2}{c}{TimeMixer} \\
         & MSE & MAE & MSE & MAE \\ \midrule
        (1) & 0.422 ± 0.001 & 0.423 ± 0.001 & 0.447 ± 0.002 & 0.440 ± 0.005 \\
        (2) & 0.355 ± 0.003 & 0.387 ± 0.001 & 0.364 ± 0.008 & 0.395 ± 0.010 \\
        (3) & 0.376 ± 0.002 & 0.388 ± 0.001 & 0.381 ± 0.003 & 0.395 ± 0.006 \\
        (4) & 0.271 ± 0.001 & 0.317 ± 0.001 & 0.275 ± 0.001 & 0.323 ± 0.003 \\
        (5) & 0.243 ± 0.001 & 0.269 ± 0.000 & 0.240 ± 0.010 & 0.271 ± 0.009 \\
        (6) & 0.177 ± 0.000 & 0.267 ± 0.000 & 0.182 ± 0.017 & 0.272 ± 0.006 \\
        (7) & 0.489 ± 0.005 & 0.297 ± 0.001 & 0.484 ± 0.015 & 0.297 ± 0.013 \\ \bottomrule
    \end{tabularx}
    \caption{Model robustness under the unified setting, including similar look-back window length, batch size, and epochs for all models. (1), (2), (3), (4), (5), (6), and (7) refer to ETTh1, ETTh2, ETTm1, ETTm2, Weather, Electricity, and Traffic datasets, respectively.}
    \label{tab:robustness}
\end{table}

==> table_unified_result_no_need_.tex <==
\begin{table*}[!htb]
    \fontsize{9}{6}\selectfont
    \begin{tabularx}{\textwidth}{@{}cccccccccccccccccccc@{}}
        \multicolumn{2}{c}{Models} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}WPMixer\\      (Ours)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}TimeMixer\\      (2024)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}iTransformer*\\      (2024)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}TSMixer\\      (2023)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}PatchTST\\      (2023)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}TimesNet\\      (2023)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Crossformer\\      (2023)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}FiLM\\      (2022a)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Dlinear\\      (2023)\end{tabular}} \\ \midrule
        \multicolumn{2}{c}{Metric} & MSE & MAE & \multicolumn{1}{l}{MSE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{MSE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{MSE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{MSE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{MSE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{MSE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{MSE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{MSE} & \multicolumn{1}{l}{MAE} \\
        \multirow{5}{*}{\begin{sideways}ETTh1\end{sideways}} & 96 & \textbf{0.368} & \textbf{0.394} & \underline{0.375} & \underline{0.400} & 0.386 & 0.405 & 0.387 & 0.411 & 0.460 & 0.447 & 0.384 & 0.402 & 0.423 & 0.448 & 0.438 & 0.433 & 0.397 & 0.412 \\
         & 192 & \textbf{0.420} & \textbf{0.418} & \underline{0.429} & \underline{0.421} & 0.441 & 0.436 & 0.441 & 0.437 & 0.512 & 0.477 & 0.436 & 0.429 & 0.471 & 0.474 & 0.493 & 0.466 & 0.446 & 0.441 \\
         & 336 & \textbf{0.452} & \textbf{0.433} & \underline{0.484} & \underline{0.458} & 0.487 & \underline{0.458} & 0.507 & 0.467 & 0.546 & 0.496 & 0.638 & 0.469 & 0.570 & 0.546 & 0.547 & 0.495 & 0.489 & 0.467 \\
         & 720 & \textbf{0.449} & \textbf{0.449} & \underline{0.498} & \underline{0.482} & 0.503 & 0.491 & 0.527 & 0.548 & 0.544 & 0.517 & 0.521 & 0.500 & 0.653 & 0.621 & 0.586 & 0.538 & 0.513 & 0.510 \\ \cmidrule{2-20}
         & Avg & \textbf{0.422} & \textbf{0.423} & \underline{0.447} & \underline{0.440} & 0.454 & 0.447 & 0.466 & 0.467 & 0.516 & 0.484 & 0.495 & 0.450 & 0.529 & 0.522 & 0.516 & 0.483 & 0.461 & 0.457 \\ \midrule
        \multirow{5}{*}{\begin{sideways}ETTh2\end{sideways}} & 96 & \textbf{0.282} & \textbf{0.334} & \underline{0.289} & \underline{0.341} & 0.297 & 0.349 & 0.308 & 0.357 & 0.308 & 0.355 & 0.340 & 0.374 & 0.745 & 0.584 & 0.322 & 0.364 & 0.340 & 0.394 \\
         & 192 & \textbf{0.359} & \textbf{0.385} & \underline{0.372} & \underline{0.392} & 0.380 & 0.400 & 0.395 & 0.404 & 0.393 & 0.405 & 0.402 & 0.414 & 0.877 & 0.656 & 0.404 & 0.414 & 0.482 & 0.479 \\
         & 336 & \textbf{0.374} & \textbf{0.404} & \underline{0.386} & \underline{0.414} & 0.428 & 0.432 & 0.428 & 0.434 & 0.427 & 0.436 & 0.452 & 0.452 & 1.043 & 0.731 & 0.435 & 0.445 & 0.591 & 0.541 \\
         & 720 & \textbf{0.405} & \textbf{0.427} & \underline{0.412} & \underline{0.434} & 0.427 & 0.445 & 0.443 & 0.451 & 0.436 & 0.450 & 0.462 & 0.468 & 1.104 & 0.763 & 0.447 & 0.458 & 0.839 & 0.661 \\ \cmidrule{2-20}
         & Avg & \textbf{0.355} & \textbf{0.387} & \underline{0.364} & \underline{0.395} & 0.383 & 0.407 & 0.394 & 0.412 & 0.391 & 0.411 & 0.414 & 0.427 & 0.942 & 0.684 & 0.402 & 0.420 & 0.563 & 0.519 \\ \midrule
        \multirow{5}{*}{\begin{sideways}ETTm1\end{sideways}} & 96 & \textbf{0.314} & \textbf{0.350} & \underline{0.320} & \underline{0.357} & 0.334 & 0.368 & 0.331 & 0.378 & 0.352 & 0.374 & 0.338 & 0.375 & 0.404 & 0.426 & 0.353 & 0.370 & 0.346 & 0.374 \\
         & 192 & \textbf{0.358} & \textbf{0.375} & \underline{0.361} & \underline{0.381} & 0.377 & 0.391 & 0.386 & 0.399 & 0.390 & 0.393 & 0.374 & 0.387 & 0.450 & 0.451 & 0.389 & 0.387 & 0.382 & 0.391 \\
         & 336 & \textbf{0.384} & \textbf{0.395} & \underline{0.390} & \underline{0.404} & 0.426 & 0.420 & 0.426 & 0.421 & 0.421 & 0.414 & 0.410 & 0.411 & 0.532 & 0.515 & 0.421 & 0.408 & 0.415 & 0.415 \\
         & 720 & \textbf{0.448} & \textbf{0.432} & \underline{0.454} & \underline{0.441} & 0.491 & 0.459 & 0.489 & 0.465 & 0.462 & 0.449 & 0.478 & 0.450 & 0.666 & 0.589 & 0.481 & \underline{0.441} & 0.473 & 0.451 \\ \cmidrule{2-20}
         & Avg & \textbf{0.376} & \textbf{0.388} & \underline{0.381} & \underline{0.395} & 0.407 & 0.410 & 0.408 & 0.416 & 0.406 & 0.407 & 0.400 & 0.406 & 0.513 & 0.495 & 0.411 & 0.402 & 0.404 & 0.408 \\ \midrule
        \multirow{5}{*}{\begin{sideways}ETTm2\end{sideways}} & 96 & \textbf{0.171} & \textbf{0.253} & \underline{0.175} & \underline{0.258} & 0.180 & 0.264 & 0.179 & 0.282 & 0.183 & 0.270 & 0.187 & 0.267 & 0.287 & 0.366 & 0.183 & 0.266 & 0.193 & 0.293 \\
         & 192 & \textbf{0.234} & \textbf{0.294} & \underline{0.237} & \underline{0.299} & 0.250 & 0.309 & 0.244 & 0.305 & 0.255 & 0.314 & 0.249 & 0.309 & 0.414 & 0.492 & 0.248 & 0.305 & 0.284 & 0.361 \\
         & 336 & \textbf{0.292} & \textbf{0.333} & \underline{0.298} & \underline{0.340} & 0.311 & 0.348 & 0.320 & 0.357 & 0.309 & 0.347 & 0.321 & 0.351 & 0.597 & 0.542 & 0.309 & 0.343 & 0.382 & 0.429 \\
         & 720 & \textbf{0.387} & \textbf{0.390} & \underline{0.391} & \underline{0.396} & 0.412 & 0.407 & 0.419 & 0.432 & 0.412 & 0.404 & 0.408 & 0.403 & 1.730 & 1.042 & 0.410 & 0.400 & 0.558 & 0.525 \\ \cmidrule{2-20}
         & Avg & \textbf{0.271} & \textbf{0.317} & \underline{0.275} & \underline{0.323} & 0.288 & 0.332 & 0.290 & 0.344 & 0.290 & 0.334 & 0.291 & 0.333 & 0.757 & 0.610 & 0.287 & 0.329 & 0.354 & 0.402 \\ \midrule
        \multirow{5}{*}{\begin{sideways}Weather\end{sideways}} & 96 & \textbf{0.162} & \textbf{0.204} & \underline{0.163} & \underline{0.209} & 0.174 & 0.214 & 0.175 & 0.247 & 0.186 & 0.227 & 0.172 & 0.220 & 0.195 & 0.271 & 0.195 & 0.236 & 0.195 & 0.252 \\
         & 192 & \underline{0.209} & \textbf{0.246} & \textbf{0.208} & \underline{0.250} & 0.221 & 0.254 & 0.224 & 0.294 & 0.234 & 0.265 & 0.219 & 0.261 & \underline{0.209} & 0.277 & 0.239 & 0.271 & 0.237 & 0.295 \\
         & 336 & 0.263 & \textbf{0.287} & \underline{0.251} & \textbf{0.287} & 0.278 & 0.296 & 0.262 & 0.326 & 0.284 & 0.301 & \textbf{0.246} & 0.337 & 0.273 & 0.332 & 0.289 & 0.306 & 0.282 & 0.331 \\
         & 720 & \textbf{0.339} & \textbf{0.338} & \textbf{0.339} & \underline{0.341} & 0.358 & 0.347 & 0.349 & 0.348 & 0.356 & 0.349 & 0.365 & 0.359 & 0.379 & 0.401 & 0.361 & 0.351 & 0.345 & 0.382 \\ \cmidrule{2-20}
         & Avg & \underline{0.243} & \textbf{0.269} & \textbf{0.240} & \underline{0.271} & 0.258 & 0.278 & 0.253 & 0.304 & 0.265 & 0.285 & 0.251 & 0.294 & 0.264 & 0.320 & 0.271 & 0.291 & 0.265 & 0.315 \\ \midrule
        \multirow{5}{*}{\begin{sideways}Electricity\end{sideways}} & 96 & \underline{0.150} & \underline{0.241} & 0.153 & 0.247 & \textbf{0.148} & \textbf{0.240} & 0.190 & 0.299 & 0.190 & 0.296 & 0.168 & 0.272 & 0.219 & 0.314 & 0.198 & 0.274 & 0.210 & 0.302 \\
         & 192 & \textbf{0.162} & \textbf{0.252} & 0.166 & 0.256 & \textbf{0.162} & \underline{0.253} & 0.216 & 0.323 & 0.199 & 0.304 & 0.184 & 0.322 & 0.231 & 0.322 & 0.198 & 0.278 & 0.210 & 0.305 \\
         & 336 & \underline{0.179} & \underline{0.270} & 0.185 & 0.277 & \textbf{0.178} & \textbf{0.269} & 0.226 & 0.334 & 0.217 & 0.319 & 0.198 & 0.300 & 0.246 & 0.337 & 0.217 & 0.300 & 0.223 & 0.319 \\
         & 720 & \textbf{0.217} & \textbf{0.304} & 0.225 & \underline{0.310} & 0.225 & 0.317 & 0.250 & 0.353 & 0.258 & 0.352 & 0.220 & 0.320 & 0.280 & 0.363 & 0.278 & 0.356 & 0.258 & 0.350 \\ \cmidrule{2-20}
         & Avg & \textbf{0.177} & \textbf{0.267} & 0.182 & 0.272 & \underline{0.178} & \underline{0.270} & 0.220 & 0.327 & 0.216 & 0.318 & 0.193 & 0.304 & 0.244 & 0.334 & 0.223 & 0.302 & 0.225 & 0.319 \\ \midrule
        \multirow{5}{*}{\begin{sideways}Traffic\end{sideways}} & 96 & 0.465 & 0.286 & \underline{0.462} & \underline{0.285} & \textbf{0.395} & \textbf{0.268} & 0.499 & 0.344 & 0.526 & 0.347 & 0.593 & 0.321 & 0.644 & 0.429 & 0.647 & 0.384 & 0.650 & 0.396 \\
         & 192 & 0.475 & \underline{0.290} & \underline{0.473} & 0.296 & \textbf{0.417} & \textbf{0.276} & 0.540 & 0.370 & 0.522 & 0.332 & 0.617 & 0.336 & 0.665 & 0.431 & 0.600 & 0.361 & 0.598 & 0.370 \\
         & 336 & \underline{0.489} & \underline{0.296} & 0.498 & \underline{0.296} & \textbf{0.433} & \textbf{0.283} & 0.557 & 0.378 & 0.517 & 0.334 & 0.629 & 0.336 & 0.674 & 0.420 & 0.610 & 0.367 & 0.605 & 0.373 \\
         & 720 & 0.527 & 0.318 & \underline{0.506} & \underline{0.313} & \textbf{0.467} & \textbf{0.302} & 0.586 & 0.397 & 0.552 & 0.352 & 0.640 & 0.350 & 0.683 & 0.424 & 0.691 & 0.425 & 0.645 & 0.394 \\ \cmidrule{2-20}
         & Avg & 0.489 & \underline{0.297} & \underline{0.484} & \underline{0.297} & \textbf{0.428} & \textbf{0.282} & 0.546 & 0.372 & 0.529 & 0.341 & 0.620 & 0.336 & 0.667 & 0.426 & 0.637 & 0.384 & 0.625 & 0.383 \\ \midrule
        \multicolumn{2}{r}{1st Cnt:} & \multicolumn{1}{c}{25} & \multicolumn{1}{c}{28} & 3 & 1 & 8 & 7 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \bottomrule
    \end{tabularx}
    \caption{Long-term Multivariate time series forecasting results with Unified setting of TimeMixer, including similar look-back window, batch size, and epochs. We optimize other hyper-parameters including learning rate, $\psi$, $m$, $t_f$, $d_f$, dropouts, Patch, Stride, and $d$. The results of the models marked with $(*)$ are taken from the corresponding original papers. Other model's results are taken from the TimeMixer\cite{c:timemixer}.}
    \label{tab:unified_result}
\end{table*}


==> table_univariate_result_no_need_.tex <==

\begin{table*}[!htb]
    \centering
    \fontsize{9}{6}\selectfont
    \begin{tabularx}{\textwidth}{cccccccccccccccccc}
        \toprule
        \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{WPMixer} & \multicolumn{2}{c}{PatchTST/64} & \multicolumn{2}{c}{PatchTST/42} & \multicolumn{2}{c}{Dlinear} & \multicolumn{2}{c}{FEDformer} & \multicolumn{2}{c}{Autoformer} & \multicolumn{2}{c}{Informer} & \multicolumn{2}{c}{LogTrans} \\ \midrule
        Data & Pred. len & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\ \midrule
        \multirow{5}{*}{ETTh1} & 96 & \textbf{0.055} & 0.181 & 0.059 & 0.189 & \textbf{0.055} & \textbf{0.179} & 0.056 & \underline{0.180} & 0.079 & 0.215 & 0.071 & 0.206 & 0.193 & 0.377 & 0.283 & 0.468 \\
         & 192 & \textbf{0.065} & \textbf{0.200} & 0.074 & 0.215 & \underline{0.071} & 0.205 & \underline{0.071} & \underline{0.204} & 0.104 & 0.245 & 0.114 & 0.262 & 0.217 & 0.395 & 0.234 & 0.409 \\
         & 336 & \textbf{0.071} & \textbf{0.212} & \underline{0.076} & \underline{0.220} & 0.081 & 0.225 & 0.098 & 0.244 & 0.119 & 0.270 & 0.107 & 0.258 & 0.202 & 0.381 & 0.386 & 0.546 \\
         & 720 & \textbf{0.083} & \textbf{0.229} & \underline{0.087} & 0.236 & \underline{0.087} & \underline{0.232} & 0.189 & 0.359 & 0.142 & 0.299 & 0.126 & 0.283 & 0.183 & 0.355 & 0.475 & 0.629 \\ \cmidrule{2-18}
         & Avg. & \textbf{0.068} & \textbf{0.205} & \underline{0.074} & 0.215 & \underline{0.074} & \underline{0.210} & 0.104 & 0.247 & 0.111 & 0.257 & 0.105 & 0.252 & 0.199 & 0.377 & 0.345 & 0.513 \\  \midrule
        \multirow{5}{*}{ETTh2} & 96 & \textbf{0.122} & \underline{0.278} & 0.131 & 0.284 & 0.129 & 0.282 & 0.131 & 0.279 & \underline{0.128} & \textbf{0.271} & 0.153 & 0.306 & 0.213 & 0.373 & 0.217 & 0.379 \\
         & 192 & \textbf{0.163} & \textbf{0.324} & 0.171 & 0.329 & \underline{0.168} & \underline{0.328} & 0.176 & 0.329 & 0.185 & 0.330 & 0.204 & 0.351 & 0.227 & 0.387 & 0.281 & 0.429 \\
         & 336 & \textbf{0.159} & \textbf{0.324} & \underline{0.171} & \underline{0.336} & 0.185 & 0.351 & 0.209 & 0.367 & 0.231 & 0.378 & 0.246 & 0.389 & 0.242 & 0.401 & 0.293 & 0.437 \\
         & 720 & \textbf{0.197} & \textbf{0.355} & \underline{0.223} & \underline{0.380} & 0.224 & 0.383 & 0.276 & 0.426 & 0.278 & 0.420 & 0.268 & 0.409 & 0.291 & 0.439 & 0.218 & 0.387 \\ \cmidrule{2-18}
         & Avg. & \textbf{0.160} & \textbf{0.320} & \underline{0.174} & \underline{0.332} & 0.177 & 0.336 & 0.198 & 0.350 & 0.206 & 0.350 & 0.218 & 0.364 & 0.243 & 0.400 & 0.252 & 0.408 \\  \midrule
        \multirow{5}{*}{ETTm1} & 96 & \textbf{0.026} & \textbf{0.121} & \textbf{0.026} & 0.123 & \textbf{0.026} & \textbf{0.121} & 0.028 & 0.123 & 0.033 & 0.140 & 0.056 & 0.183 & 0.109 & 0.277 & 0.049 & 0.171 \\
         & 192 & \textbf{0.038} & \textbf{0.149} & 0.040 & 0.151 & \underline{0.039} & \underline{0.150} & 0.045 & 0.156 & 0.058 & 0.186 & 0.081 & 0.216 & 0.151 & 0.310 & 0.157 & 0.317 \\
         & 336 & \textbf{0.051} & \textbf{0.172} & \underline{0.053} & 0.174 & \underline{0.053} & \underline{0.173} & 0.061 & 0.182 & 0.084 & 0.231 & 0.076 & 0.218 & 0.427 & 0.591 & 0.289 & 0.459 \\
         & 720 & \textbf{0.068} & \textbf{0.197} & \underline{0.073} & \underline{0.206} & 0.074 & 0.207 & 0.080 & 0.210 & 0.102 & 0.250 & 0.110 & 0.267 & 0.438 & 0.586 & 0.43 & 0.579 \\  \cmidrule{2-18}
         & Avg. & \textbf{0.046} & \textbf{0.160} & \underline{0.048} & 0.164 & \underline{0.048} & \underline{0.163} & 0.054 & 0.168 & 0.069 & 0.202 & 0.081 & 0.221 & 0.281 & 0.441 & 0.231 & 0.382 \\  \midrule
        \multirow{5}{*}{ETTm2} & 96 & \textbf{0.063} & \underline{0.184} & 0.065 & 0.187 & 0.065 & 0.186 & \textbf{0.063} & \textbf{0.183} & 0.067 & 0.198 & 0.065 & 0.189 & 0.088 & 0.225 & 0.075 & 0.208 \\
         & 192 & \underline{0.093} & \underline{0.229} & \underline{0.093} & 0.231 & 0.094 & 0.231 & \textbf{0.092} & \textbf{0.227} & 0.102 & 0.245 & 0.118 & 0.256 & 0.132 & 0.283 & 0.129 & 0.275 \\
         & 336 & \textbf{0.118} & \underline{0.263} & 0.121 & 0.266 & 0.120 & 0.265 & \underline{0.119} & \textbf{0.261} & 0.130 & 0.279 & 0.154 & 0.305 & 0.180 & 0.336 & 0.154 & 0.302 \\
         & 720 & \textbf{0.166} & \textbf{0.318} & 0.172 & 0.322 & \underline{0.171} & 0.322 & 0.175 & \underline{0.320} & 0.178 & 0.325 & 0.182 & 0.335 & 0.300 & 0.435 & 0.16 & 0.321 \\  \cmidrule{2-18}
         & Avg. & \textbf{0.110} & \underline{0.249} & 0.113 & 0.252 & 0.113 & 0.251 & \underline{0.112} & \textbf{0.248} & 0.119 & 0.262 & 0.130 & 0.271 & 0.175 & 0.320 & 0.130 & 0.277 \\ \bottomrule
    \end{tabularx}
    \caption{Univariate Long-term time series prediction result. The results of the other models are directly taken from PatchTST \cite{c:patchtst}.}
    \label{tab:univariate_result}
\end{table*}
